PosterO: Structuring Layout Trees to Enable Language Models in Generalized Content-Aware Layout Generation

In poster design, content-aware layout generation is crucial for automatically arranging visual-textual elements on the given image. With limited training data, existing work focused on image-centric enhancement. However, this neglects the diversity of layouts and fails to cope with shape-variant elements or diverse design intents in generalized settings. To this end, we proposed a layout-centric approach that leverages layout knowledge implicit in large language models (LLMs) to create posters for omnifarious purposes, hence the name PosterO. Specifically, it structures layouts from datasets as trees in SVG language by universal shape, design intent vectorization, and hierarchical node representation. Then, it applies LLMs during inference to predict new layout trees by in-context learning with intent-aligned example selection. After layout trees are generated, we can seamlessly realize them into poster designs by editing the chat with LLMs. Extensive experimental results have demonstrated that PosterO can generate visually appealing layouts for given images, achieving new state-of-the-art performance across various benchmarks. To further explore PosterO's abilities under the generalized settings, we built PStylish7, the first dataset with multi-purpose posters and various-shaped elements, further offering a challenging test for advanced research.

==> sec/old-4_experiments.tex <==
\section{Experiment}
\label{sec:experiment}



\subsection{Evaluation Metrics}

\begin{table}[t]
\resizebox{\linewidth}{!}
{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{0}{Metrics}        & \multicolumn{2}{c}{PKU}           & \multicolumn{2}{c}{CGL}           \\ \cmidrule(lr{0pt}){2-3} \cmidrule(lr{0pt}){4-5}
               & Match $\uparrow$ & Unmatch $\downarrow$ & Match $\uparrow$ & Unmatch $\downarrow$ \\ \midrule
Saliency map & 0.22383        & 0.11926          & 0.19842        & 0.13522          \\
Density map  & \textbf{0.44142}        & \textbf{0.09957}          & \textbf{0.40364}        & \textbf{0.08831}          \\ 
      & (+0.2176)      & (-0.0197)        & (+0.2052)      & (-0.0469)        \\ \bottomrule
\end{tabular}
}

\resizebox{\linewidth}{!}
{
\begin{tabular}{lccc}
Costs          & Architecture   & \#FLOPs(G)    & \#Params(M)     \\ \midrule
Saliency model & ISNet + BASNet & 287.83        & 131.11          \\
Density model  & UNet (MiT-B1)  & \textbf{3.74} & \textbf{16.43}  \\
\bottomrule
\end{tabular}
}
\caption{Comparisons of metric effectiveness and model efficiency between the saliecny and density paradigms on the \textit{annotated test} split (Real data) of PKU PosterLayout and CGL datasets.}
\label{tab:sal_vs_den}
\end{table}

\subsection{Implementation Details}


\subsection{Comparison with State-of-the-arts}



\begin{table*}[t]
    \centering
    \begin{tabular}{l|llll|lllll} \toprule
Method &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\
\midrule
\textit{\small Training-based}     &        &        &        &        &        &        &        &        &        \\
CGL-GAN                            & 0.1010 & 0.0048 & 0.7326 & 0.2743 & 0.1693 & 0.2105 & 0.0327 & \uline{0.3573} & 0.0949 \\
DS-GAN                             & \uline{0.0248} & \uline{0.0046} & \uline{0.7859} & \uline{0.4676} & \textbf{0.1832} & 0.1894 & 0.0320 & \textbf{0.3661} & 0.1032 \\
ICVT                               & 0.2786 & 0.0480 & 0.4939 & \uline{0.3549} & 0.1050 & 0.2686 & 0.0347 & 0.1752 & \uline{0.0708} \\
LayoutDM\dag                       & 0.1638 & \textbf{0.0029} & 0.5987 & 0.3695 & \uline{0.1475} & \uline{0.1504} & \uline{0.0264} & 0.2950 & 0.0751 \\
RALF                               & \textbf{0.0175} & 0.0069 & \textbf{0.9548} & \textbf{0.8653} & 0.1452 & \textbf{0.1328} & \textbf{0.0231} & 0.2871 & \textbf{0.0701} \\
\midrule
\textit{\small Tuning-based VLM} &        &        &        &        &        &        &        &        &        \\
PosterLLaMa\ddag                 & 0.0006 & 0.0006 & 0.9986 & 0.9917 & 0.1764 & 0.1630 & 0.0285 & 0.3343 & 0.0951 \\
% PosterLLaVa\dag                    & 0.0001 & 0.0002 & 1.0000 & 1.0000 & 0.2628 & 0.1649 & 0.0249 &        &        \\
\midrule
\textit{\small Tuning-free   LLM}  &        &        &        &        &        &        &        &        &        \\
LayoutPrompter$_{L2}$   & 0.0095 & 0.0032 & 0.3401 & 0.1161 & 0.1588 & 0.2619 & 0.0408 & 0.2594 & 0.1210 \\
LayoutPrompter$_{CL}$   & 0.0032 & 0.0028 & 0.4052 & 0.1464 & 0.1713 & 0.2522 & 0.0395 & 0.2884 & 0.1243 \\
LayoutPrompter$_{L3.1}$ & 0.0010 & 0.0026 & 0.4054 & 0.1621 & \textbf{0.2025} & 0.2539 & 0.0412 & 0.3297 & 0.1507 \\
PosterO$_{L2}$ (Ours)   & \uline{0.0005} & 0.0029 & 0.7228 & 0.5073 & 0.1580 & \uline{0.1494} & 0.0268 & 0.3043 & \textbf{0.0842} \\
PosterO$_{CL}$ (Ours)   & \textbf{0.0004} & \uline{0.0027} & \uline{0.9592} & \uline{0.8243} & 0.1689 & 0.1579 & \uline{0.0265} & \uline{0.3290} & \uline{0.0917} \\
PosterO$_{L3.1}$ (Ours) & \uline{0.0005} & \textbf{0.0025} & \textbf{0.9873} & \textbf{0.9250} & \uline{0.1882} & \textbf{0.1422} & \textbf{0.0244} & \textbf{0.3710} & 0.0986 \\
\bottomrule
    \end{tabular}
    \caption{Comparisons on the \textit{unannotated test} split of PKU PosterLayout Dataset.}
    \label{tab:unan_pku}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|llll|lllll} \toprule
Method &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\ \midrule
\textcolor{gray!60}{\textit{Real data}}    & \textcolor{gray!60}{0.0010} & \textcolor{gray!60}{0.0038} & \textcolor{gray!60}{0.9942} & \textcolor{gray!60}{0.9903} & \textcolor{gray!60}{0.2238} & \textcolor{gray!60}{0.1193} & \textcolor{gray!60}{0.0109} & \textcolor{gray!60}{0.4414} & \textcolor{gray!60}{0.0996} \\
\textit{\small Training-based}    &        &        &        &        &        &        &        &        \\
CGL-GAN                           & 0.0966 & 0.0035 & 0.7854 & 0.3570 & 0.2065 & 0.1548 & 0.0191 & \textbf{0.4529} & 0.0901 \\
DS-GAN                            & \uline{0.0261} & 0.0038 & \uline{0.8350} & \uline{0.5804} & \uline{0.2078} & 0.1591 & 0.0199 & \uline{0.4428} & 0.0954 \\
ICVT                              & 0.2572 & 0.0405 & 0.5384 & 0.3932 & 0.1161 & 0.2401 & 0.0259 & 0.2159 & \textbf{0.0645} \\
LayoutDM\dag                      & 0.1562 & \textbf{0.0018} & 0.6426 & 0.3873 & 0.1600 & \uline{0.1432} & \uline{0.0185} & 0.3443 & \uline{0.0690} \\
RALF                              & \textbf{0.0084} & \uline{0.0028} & \textbf{0.9808} & \textbf{0.9201} & \textbf{0.2137} & \textbf{0.1195} & \textbf{0.0128} & 0.4308 & 0.0927 \\
\midrule
\textit{\small Tuning-based VLM}  &        &        &        &        &        &        &        &        &        \\
PosterLLaMa\ddag                  & 0.0008 & 0.0006 & 0.9999 & 0.9982 & 0.1812 & 0.1489 & 0.0177 & 0.3718 & 0.0807 \\
\midrule
\textit{\small Tuning-free   LLM}  &        &        &        &        &        &        &        &        &        \\
LayoutPrompter$_{L2}$   & 0.0083 & 0.0030 & 0.3716 & 0.1633 & 0.1615 & 0.2300 & 0.0319 & 0.2827 & 0.1035 \\
LayoutPrompter$_{CL}$   & 0.0040 & 0.0030 & 0.4415 & 0.1937 & 0.1838 & 0.2286 & 0.0301 & 0.3290 & 0.1167 \\
LayoutPrompter$_{L3.1}$ & \uline{0.0017} & 0.0028 & 0.4085 & 0.1613 & \textbf{0.2104} & 0.2271 & 0.0309 & 0.3606 & 0.1381 \\
PosterO$_{L2}$ (Ours)   & \textbf{0.0005} & 0.0029 & 0.7571 & 0.5664 & 0.1771 & \textbf{0.1312} & \uline{0.0176} & 0.3467 & \textbf{0.0810} \\
PosterO$_{CL}$ (Ours)   & \textbf{0.0005} & \uline{0.0027} & \uline{0.9732} & \uline{0.8859} & 0.1878 & 0.1415 & 0.0178 & \uline{0.3732} & \uline{0.0866} \\
PosterO$_{L3.1}$ (Ours) & \textbf{0.0005} & \textbf{0.0024} & \textbf{0.9886} & \textbf{0.9363} & \uline{0.2026} & \uline{0.1334} & \textbf{0.0170} & \textbf{0.4059} & 0.0915 \\
\bottomrule
    \end{tabular}
    \caption{Comparisons on the \textit{annotated test} split of PKU PosterLayout Dataset.}
    \label{tab:an_pku}
\end{table*}

\begin{table*}[t]
\centering
{
    \begin{tabular}{l|llll|lllll}
\toprule
Method &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\
\midrule
\textit{\small Training-based}     &        &        &        &        &        &        &        &        &        \\
CGL-GAN                            & 0.2668 & 0.0316 & 0.6774 & 0.1656 & 0.0554 & 0.4312 & \uline{0.0512} & \uline{0.1217} & 0.0446 \\
DS-GAN                             & 0.0991 & \uline{0.0138} & \uline{0.7566} & 0.2810 & \textbf{0.1339} & \uline{0.4277} & 0.0526 & \textbf{0.2561} & 0.1062 \\
ICVT                               & 0.2045 & 0.1010 & 0.4357 & 0.2599 & 0.0360 & 0.4620 & \textbf{0.0397} & 0.0566 & \uline{0.0269} \\
LayoutDM\dag                       & \uline{0.0793} & 0.1822 & 0.6304 & \uline{0.3853} & 0.0131 & 0.5438 & 0.0612 & 0.0207 & \textbf{0.0130} \\
RALF                               & \textbf{0.0273} & \textbf{0.0189} & \textbf{0.9756} & \textbf{0.9315} & \uline{0.0601} & \textbf{0.3359} & \textbf{0.0397} & 0.1042 & 0.0425 \\
% CGB-DM                             &        &        &        &        &        &        &        &        &        \\
\midrule
\textit{\small Tuning-based VLM}  &        &        &        &        &        &        &        &        &        \\
PosterLLaMa\ddag                  & 0.0014 & 0.0007 & 0.9971 & 0.9771 & 0.1032 & 0.4687 & 0.0555 & 0.2024 & 0.0886 \\
\midrule
\textit{\small Tuning-free   LLM}  &        &        &        &        &        &        &        &        &        \\
LayoutPrompter$_{L2}$   & 0.0069 & 0.0103 & 0.2847 & 0.1126 & 0.1458 & 0.4427 & 0.0628 & 0.1802 & 0.1446 \\
LayoutPrompter$_{CL}$   & 0.0045 & \uline{0.0024} & 0.3239 & 0.1341 & \uline{0.1919} & 0.4729 & 0.0650 & 0.2399 & 0.2021 \\
LayoutPrompter$_{L3.1}$ & 0.0026 & \textbf{0.0016} & 0.2693 & 0.1142 & \textbf{0.2008} & 0.4570 & 0.0644 & 0.2394 & 0.2060 \\
PosterO$_{L2}$ (Ours)   & 0.0005 & 0.0033 & 0.6663 & 0.4770 & 0.1371 & \textbf{0.2893} & 0.0382 & 0.2334 & \uline{0.0933} \\
PosterO$_{CL}$ (Ours)   & \textbf{0.0003} & 0.0037 & \uline{0.9369} & \uline{0.8071} & 0.1344 & 0.3004 & \uline{0.0379} & \uline{0.2533} & \textbf{0.0897} \\
PosterO$_{L3.1}$ (Ours) & \uline{0.0004} & 0.0032 & \textbf{0.9816} & \textbf{0.9034} & 0.1641 & \uline{0.2944} & \textbf{0.0365} & \textbf{0.2974} & 0.1099 \\
\bottomrule
    \end{tabular}
}
    \caption{Comparisons on the \textit{unannotated test} split of CGL Dataset.}
    \label{tab:unan_cgl}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|llll|lllll}
\toprule
Method &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\
\midrule
\textcolor{gray!60}{\textit{Real data}} & \textcolor{gray!60}{0.0003} & \textcolor{gray!60}{0.0024} & \textcolor{gray!60}{0.9963} & \textcolor{gray!60}{0.9880} & \textcolor{gray!60}{0.1984} & \textcolor{gray!60}{0.1352} & \textcolor{gray!60}{0.0119} & \textcolor{gray!60}{0.4036} & \textcolor{gray!60}{0.0883} \\
\textit{\small Training-based}    &        &        &        &        &        &        &        &        &        \\
CGL-GAN                           & 0.2291 & 0.0123 & 0.6466 & 0.2281 & 0.1096 & 0.1811 & 0.0213 & 0.2491 & \textbf{0.0487} \\
DS-GAN                            & 0.0460 & \uline{0.0022} & 0.9081 & 0.6308 & \textbf{0.2408} & 0.1476 & 0.0181 & \textbf{0.5012} & 0.1084 \\
ICVT                              & \textbf{0.2453} & 0.0179 & 0.5150 & 0.3326 & 0.1488 & 0.1945 & 0.0211 & 0.3040 & \uline{0.0710} \\
LayoutDM\dag                      & \uline{0.0184} & \textbf{0.0021} & \uline{0.9216} & \uline{0.8159} & 0.1933 & \uline{0.1369} & \textbf{0.0137} & 0.3948 & 0.0859 \\
RALF                              & \textbf{0.0042} & 0.0024 & \textbf{0.9912} & \textbf{0.9756} & \uline{0.1969} & \textbf{0.1246} & \uline{0.0180} & \uline{0.4003} & 0.0854 \\
% CGB-DM                            &        &        &        &        &        &        &        &        &        \\
\midrule
\textit{\small Tuning-based VLM}  &        &        &        &        &        &        &        &        &        \\
PosterLLaMa\ddag                  & 0.0006 & 0.0006 & 0.9987 & 0.9890 & 0.1775 & 0.1647 & 0.0184 & 0.3732 & 0.0809 \\
\midrule
\textit{\small Tuning-free   LLM}  &        &        &        &        &        &        &        &        &        \\
LayoutPrompter$_{L2}$   & 0.0087 & 0.0033 & 0.3369 & 0.1455 & 0.1454 & 0.2354 & 0.0327 & 0.2583 & 0.0956 \\
LayoutPrompter$_{CL}$   & 0.0037 & 0.0031 & 0.3965 & 0.1616 & 0.1620 & 0.2323 & 0.0317 & 0.2933 & 0.1039 \\
LayoutPrompter$_{L3.1}$ & 0.0017 & 0.0030 & 0.3830 & 0.1740 & \uline{0.1835} & 0.2380 & 0.0327 & 0.3183 & 0.1241 \\
PosterO$_{L2}$ (Ours)   & \uline{0.0006} & \uline{0.0023} & 0.7801 & 0.6150 & 0.1671 & \textbf{0.1330} & 0.0176 & 0.3386 & \textbf{0.0755} \\
PosterO$_{CL}$ (Ours)   & \textbf{0.0005} & \uline{0.0023} & \uline{0.9682} & \uline{0.8868} & 0.1809 & 0.1404 & \uline{0.0168} & \uline{0.3734} & \uline{0.0817} \\
PosterO$_{L3.1}$ (Ours) & \uline{0.0006} & \textbf{0.0022} & \textbf{0.9842} & \textbf{0.9340} & \textbf{0.2006} & \uline{0.1341} & \textbf{0.0161} & \textbf{0.4116} & 0.0904 \\
\bottomrule
    \end{tabular}
    \caption{Comparisons on the \textit{annotated test} split of CGL Dataset.}
    \label{tab:an_cgl}
\end{table*}

\subsection{Ablation Study}

\begin{table*}[t]
    \centering
    \begin{tabular}{cc|llll|llllll}
\toprule
  S &
  C &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\
\midrule
        &         & 0.0699 & 0.0039 & 0.6362 & 0.4919 & 0.4473 & 0.2403 & 0.0354 & 0.6353 & 0.3539 \\
        & $\surd$ & 0.0203 & 0.0043 & 0.7321 & 0.5433 & 0.2514 & 0.2120 & 0.0321 & 0.4011 & 0.1816 \\
$\surd$ &         & 0.1192 & 0.0043 & 0.9121 & 0.8083 & 0.3991 & 0.2258 & 0.0339 & 0.5547 & 0.3093 \\
$\surd$ & $\surd$ & 0.0972 & 0.0036 & 0.9625 & 0.8665 & 0.2275 & 0.2160 & 0.0329 & 0.3390 & 0.1689 \\
\bottomrule
    \end{tabular}
    \caption{Ablation on the structured (S) and conditioned (C) strategies for generating layout descriptions.}
\end{table*}

\begin{table*}[t]
    \centering
    \begin{tabular}{l|llll|lllll} \toprule
Backbone &
  $Ove \downarrow$ &
  $Ali \downarrow$ &
  $Und_l \uparrow$ &
  $Und_s \uparrow$ &
  $Uti \uparrow$ &
  $Occ \downarrow$ &
  $Rea \downarrow$ &
  $Cov \uparrow$ &
  $Con \downarrow$ \\ \midrule
\textcolor{gray!60}{\textit{Real data}}    & \textcolor{gray!60}{0.0010} & \textcolor{gray!60}{0.0038} & \textcolor{gray!60}{0.9942} & \textcolor{gray!60}{0.9903} & \textcolor{gray!60}{0.2238} & \textcolor{gray!60}{0.1193} & \textcolor{gray!60}{0.0109} & \textcolor{gray!60}{0.4414} & \textcolor{gray!60}{0.0996} \\
$3.1$-8B & \textbf{0.0005} & \textbf{0.0024} & \textbf{0.9886} & \textbf{0.9363} & \uline{0.2026} & \uline{0.1334} & \textbf{0.0170} & \textbf{0.4059} & 0.0915 \\
$3.2$-3B & 0.0005 & 0.0026 & 0.9731 & 0.8786 & 0.1951 & 0.1389 & 0.0184 & 0.3852 & 0.0903 \\
$3.2$-1B & 0.0007 & 0.0027 & 0.9014 & 0.6767 & 0.1898 & 0.1391 & 0.0192 & 0.3698 & 0.0883 \\
\bottomrule
    \end{tabular}
    \caption{More results on PKU PosterLayout Dataset.}
    \label{tab:more_pku}
\end{table*}
